Estimation of Building Energy Demand Characteristics using Bayesian Statistics and Energy Signature Models

This work presents a scalable Bayesian modeling framework for evaluating building energy performance using smart-meter data from 2,788 Danish single-family homes. The framework leverages Bayesian statistical inference integrated with Energy Signature (ES) models to characterize thermal performance in buildings. This approach quantifies key parameters such as the Heat Loss Coefficient (HLC), solar gain, and wind infiltration, while providing full posterior distributions to reflect parameter uncertainty. Three model variants are developed: a baseline ES model, an auto-regressive model (ARX-ES) to account for thermal inertia, and an auto-regressive moving average model (ARMAX-ES) that approximates stochastic gray-box dynamics. Results show that model complexity improves one-step-ahead predictive performance, with the ARMAX-ES model achieving a median Bayesian R^2 of 0.94 across the building stock. At the single-building level, the Bayesian approach yields credible intervals for yearly energy demand within $\pm1\%$, enabling more robust diagnostics than deterministic methods. Beyond improved accuracy, the Bayesian framework enhances decision-making by explicitly representing uncertainty in building performance parameters. This provides a more realistic foundation for investment prioritization, demand forecasting, and long-term energy planning. The method is readily applicable to other building typologies or geographies, offering a scalable tool for data-driven energy management under uncertainty.

==> Sections/1_old_Bayes.tex <==

By contrast, Bayesian statistics offers an alternative approach to traditional Frequentist approach \cite{GRILLONE2020110027}. In Bayesian framework, the goal is not to estimate a single parameter value to maximise predictive performance, but the parameter's entire probability distribution - resulting in a more robust and informative models.

Bayesian approach provides several key advantages, particularly in their ability to incorporate prior expert knowledge about building physics - such as heat transfer principles, insulation properties, and typical building materials - into the modeling process of a given building stock. By doing so, Bayesian models remain grounded in the physical realities of buildings, even when the data available is noisy or incomplete.

The most promising feature of the Bayesian approach is its capacity to directly quantify uncertainty. Unlike typical methods, which yield confidence intervals that tend shrink with more data regardless of weather the model assumptions are correct. Bayesian method provide credibility intervals that reflect the true level of uncertainty about model parameters, such as Heat Loss Coefficient (HLC). This capability is particularly important for decision-making in the building and energy sector, as it ensures that the model remains realistic and robust in the presence of inherent uncertainty.

In building energy modelling, this additional information is crucial for better understanding the inherent variability in energy performance across the building stock, providing stakeholders—such as building engineers, owners, and energy providers—with actionable insights. These insights allow creation of more accurate and robust forecasting models, better energy efficiency planning, and improved understanding of extreme user behaviors.

Despite these advantages, the Bayesian approach is computationally intensive, as it requires sampling from posterior distributions, often via Markov Chain Monte Carlo (MCMC) methods. While this adds complexity to the modeling process, the benefits of the probabilistic interpretation and the ability to integrate prior knowledge outweigh the computational burden in many applications, as will be evident from this paper.

Particularly novel aspect of Bayesian statistics, how it can enhance insights provided by established energy-demand models. The focus of this paper is the application of Bayesian framework on Energy Signature models and its extensions.


\subsubsection{Why Bayesian?}

In contrast to typical (frequentist) statistical methods, which provide point estimates and confidence intervals, Bayesian methods use credibility intervals to express uncertainty. A key advantage of Bayesian inference is that it treats model parameters as distributions rather than fixed values, allowing to describe a range of possible outcomes rather than single estimates. This is especially useful in contexts like building energy modeling where the data is often noisy and precise parameter estimates are difficult to obtain.

One of the most valuable features of Bayesian modeling is the ability to incorporate prior expert knowledge directly into the model through the use of priors. This is particularly important in cross-disciplinary domains such as building energy modelling, where physical laws govern much of the system behaviour. By integrating this expert knowledge, we can ensure that the model remains physically realistic even when the data is sparse or noisy. 

For example, in building heat demand models, prior knowledge about the heat transfer principles, insulation properties, and building materials can be encoded as parameter priors such as the reasonable HLC values for given building population. These priors act as a guide for the model, constraining it to physically reasonable values, which is crucial when working with real-world systems that are often complex and noisy. This ensures that the model's outputs are grounded in reality and align with established principles of thermodynamics and heat-flow.

\paragraph{Directly Quantifying Uncertainty}

Bayesian methods sample from the posterior distribution - $ p(\theta | X)$, which represents the probability of different model parameter values after observing the data. This approach is more realistic than simply providing point estimates, as it allows decision-makes (stakeholders?) to understant the full range of possible outcomes and how likely they are. E.g. A posterior probability distribution of the HLC, for instance, provides insight into how likely various values are, offering a clearer picture of a building's thermal performance, even in the presence of incomplete or uncertain data. (Alternatively: )

A common pitfall of regular (frequentist) approaches is that they often provide overly confident confidence intervals, especially when assumptions are made on the underlying parameter estimate distributions. In frequentist approaches, the CIs tend to shrink asymptotically as more data is added, even the the assumptions (such as normally distributed errors or linear relationships) are not valid. This in turn leads to overconfidence in model's predictions and parameter estimates. For instance, in building energy modelling, frequentist models may underestimate the uncertainty of parameters like the HLC, leading to misleadingly narrow CIs. In practice, this can result in poor decisions regarding building upgrades or energy saving strategies.

\paragraph{Computational Intensity and Drawbacks}

The Bayesian approach is not without its drawbacks. One of the most significant challenges is the computations intensity required to fit complex models on large datasets. Unlike frequentist methods, which typically involve straightforward optimisation techniques, Bayesian methods require sampling from posterior distribution. This often involves Markov Chain Monte Carlo (MCMC) simulations or similar sampling algorithms, which are computationally demanding especially for large datasets or complex models. 

In the context of building energy modelling, this computational burden can be a limitation when working with high-frequency data (e.g. from smart meters). For this reason, in this paper, the models are fitted to daily-average heat demand data, which provides enough complexity to convey key building characteristics and results of these models can be used to inform more complex forecasting models built on hourly observations. 

